Wavelet regression and additive models for irregularly spaced data

We present a novel approach for nonparametric regression using wavelet basis functions. Our proposal, $\texttt{waveMesh}$, can be applied to non-equispaced data with sample size not necessarily a power of 2. We develop an efficient proximal gradient descent algorithm for computing the estimator and establish adaptive minimax convergence rates. The main appeal of our approach is that it naturally extends to additive and sparse additive models for a potentially large number of covariates. We prove minimax optimal convergence rates under a weak compatibility condition for sparse additive models. The compatibility condition holds when we have a small number of covariates. Additionally, we establish convergence rates for when the condition is not met. We complement our theoretical results with empirical studies comparing $\texttt{waveMesh}$ to existing methods.

==> sections/realdata.tex <==
% !TeX root = ../Manuscript.tex

\section{Analysis of real world data}
\label{sec:realData}

\subsection{Analysis of simulated motorcycle accident data}
\label{sec:realdataUNI}

    

